Certifying Counterfactual Bias in LLMs

Large Language Models (LLMs) can produce biased responses that can cause representational harms. However, conventional studies are insufficient to thoroughly evaluate biases across LLM responses for different demographic groups (a.k.a. counterfactual bias), as they do not scale to large number of inputs and do not provide guarantees. Therefore, we propose the first framework, LLMCert-B that certifies LLMs for counterfactual bias on distributions of prompts. A certificate consists of high-confidence bounds on the probability of unbiased LLM responses for any set of counterfactual prompts - prompts differing by demographic groups, sampled from a distribution. We illustrate counterfactual bias certification for distributions of counterfactual prompts created by applying prefixes sampled from prefix distributions, to a given set of prompts. We consider prefix distributions consisting random token sequences, mixtures of manual jailbreaks, and perturbations of jailbreaks in LLM's embedding space. We generate non-trivial certificates for SOTA LLMs, exposing their vulnerabilities over distributions of prompts generated from computationally inexpensive prefix distributions.

==> contents/checklist.tex <==
\newpage
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}%, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our claims match our evaluation results and we have conducted case studies to provide further validation of our claims. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have an explicit limitations section to discuss them. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have clearly stated the assumptions of our theoretical framework. As our work leverages existing theoretical results, we provide appropriate references needed to understand our framework in detail. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we provide all the details in our paper and code. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the code for the project. We use open-source datasets for our experiments.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We state our experimental setup in Section~\ref{sec:results}. We list our hyperparameters in Table~\ref{tab:hyperparameters} and perform an ablation study on them in Appendix~\ref{app:hyperparams}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper states the confidence with which our results hold, i.e., $95\%$. As we have a framework based on confidence intervals, we satisfy this requirement in all our results. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: These details are mentioned in Section~\ref{sec:results}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We use open-sourced datasets in our experiments. Our work is about certifying the bias in LLMs, thus requiring us to use prompts that can elicit bias in a common setting. We warn the readers in the abstract about offensive content in the paper. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the broader impacts of our work in the Appendix~\ref{app:impacts}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not contribute new models or datasets. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have included appropriate citations and have adhered to the licenses. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the code to replicate our main results. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The supplementary material provides the HTML file to render the full set of instructions given to Amazon Mechanical Turkers to evaluate our bias metric. We provide the details in Appendix~\ref{app:biasmetrics}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our only experiment with human subjects was a crowd-sourcing experiment on Amazon Mechanical Turk, which we describe in Appendix~\ref{app:biasmetrics}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> contents/limitations.tex <==
\section{Limitations and Future Work}

\textit{Dependence on the bias detector}. The certification outcomes of \tool{} highly depend on the quality of the bias detector. The dependence is lesser than that for methods in benchmarking and adversarial example generation, as certification is based on several examples, that smooth out the noise in the bias detection function. However, this dependence on the metric can introduce cases where the certificate can appear counterintuitive. This suggests $2$ orthogonal lines of future work --- developing more human-aligned bias detectors, and certifiers robust to the noise in bias detectors. 

\textit{Scaling with hyperparameters}. \tool{}'s sample complexity can rise significantly for higher confidence requirements. To combat this, we plan to devise few-shot certification methods, that can leverage the internals of the LLMs to reduce the certification overhead. 

% Other directions of future work include developing fair LLMs by construction. This objective can specifically leverage insights from~\citep{dwork2011fairness}. 


% \todo{mention developing fair LLMs by design using Dwork et al}

==> contents/rough.tex <==
\section{Certificate generation}
We develop a general framework to quantitatively certify the bias in the responses of Large Language Models (LLMs) used as chatbots. Specifically, our certificate captures the average case bias in the model and does not take worst-case, adversarial cases into account. We generate certificates for the bias exhibited by the target LLM when prompted with a spectrum of prompting schemes. 
An instance of bias is when the responses generated by an LLM for a set of similar prompts, each corresponding to a specific instance of a given sensitive attribute, have an asymmetry in them owing to the sensitive attribute~\cite{helm}. 

\subsection{Bias specification}

We next formalize the above definition to form a specification for bias certification. Consider a given sensitive attribute $\attr$ that has $\numattr>1$ unique instances, $\attr_1,\dots,\attr_\numattr$. 
Let $\promptspace$ be the set of all input prompts to the target LLM $\llm$ and $\prompts=\{\prompts_1,\dots\prompts_\numprompts\}$ be a set of prompts, $\prompts_i\in\promptspace$, where each corresponds to a different sensitive attribute in $\attr$ and every instance of $\attr$ is covered 
The set of prompts $\prompts$ qualify to be considered in the certification process, if and only if (iff) they satisfy the precondition in Equation~\eqref{eq:precondition}, 
where $\promptdist:\promptspace\times\promptspace\rightarrow\mathbb{R}$ is a user-defined distance function between a given pair of prompts that measures the closeness of a pair of prompts, discounting for the specific instance of $\attr$ present in each of them and $\epsilon>0$ is a small constant which is the maximum permissible distance between a given pair of prompts. Intuitively, the precondition~\eqref{eq:precondition} allows the set of prompts where each pair of prompts is similar (as measured by $\promptdist$ and $\epsilon$) except for the sensitive attribute of the prompt. 

\begin{equation}
    \label{eq:precondition}
    \varphi(\prompts) = \forall p,q \in \prompts\ldotp\promptdist(p, q) < \epsilon
\end{equation}

We generate the certificate only for the set of prompts $\prompts$ that satisfy the precondition~\eqref{eq:precondition}. Each prompt in such sets is individually given to the target LLM $\llm$ (each in fresh chat instances) and the obtained responses, $\response = \{\response_1,\dots\response_\numattr\}$, each of which belong to the space of all possible responses of the LLM, $\outputspace$, are checked for bias. 
Specifically, the user defines a bias measurement function $\biasmeas$ that measures the disparity in the obtained responses for the different sensitive attributes.
% Let denote the bias measurement function. 
Then the responses $\response$ of $\llm$ are certified to be unbiased for the given set of prompts $\prompts$ if the postcondition in Equation~\eqref{eq:postcondition} is satisfied, where $\delta>0$ is a small constant that denotes the permissible amount of the bias in $\llm$'s responses.

\begin{equation}
    \label{eq:postcondition}
    \psi(\response) \triangleq \biasmeas(\response) < \delta 
\end{equation}


Hence, we define our certificate as whether for the set of prompts on which the precondition~\eqref{eq:precondition} holds, the postcondition holds on the responses generated by the target LLM. The certification is modulo $\promptdist, \biasmeas$. 

Generating the bias certificate for all sets of prompts that satisfy the precondition is infeasible as there can be infinitely many such sets. Hence, we scope down the certificate to a local certificate, wherein the set of prompts is derived from a base prompt $\prompts_0$ such that each has a different sensitive attribute and the set satisfies the precondition. Moreover, as the number of sets of local prompts that satisfy the precondition is large and not represented in closed-form, and as LLMs are stochastic text generators, we derive the probability of unbiased response from the LLM and bound it by some small constant permissible-bias threshold $\eta\geq0$. This probability is derived with a given conditional distribution $\dist(\prompts_0,\attr)$ defined over the joint sample space of $\numattr$ prompts each corresponding to different values of $\attr$ in the local region of the base prompt $\prompts_0$ that satisfies the precondition. The overall local probabilistic certification problem thus becomes the truth value of $\cert(\prompts_0,\attr)$ defined in Equation~\ref{eq:certprob}.

\begin{equation}
    \label{eq:certprob}
    \cert(\prompts_0,\attr) \triangleq Pr_{\prompts\sim\dist(\prompts_0,\attr)}[\psi(\response)] \geq 1-\eta 
\end{equation}

\subsection{Certification algorithm}\label{sec:cp}
Our certification algorithm determines $\cert(\prompts_0,\attr)$~\eqref{eq:certprob} for any given $\prompts_0$ with high confidence. We use the Clopper-Pearson confidence intervals~\cite{clopper-pearson} of the probability term in \eqref{eq:certprob} to determine the certificate. 
Next, we describe the Clopper-Pearson confidence intervals briefly and refer the interested readers to a more detailed explanation in \citep{clopper-pearson, cp_ref, cp_ref2, cp_ref3}. 

Clopper-Pearson confidence intervals provide lower and upper bounds on the probability of success parameter of a binomial random variable with probabilistic guarantees. The confidence intervals obtained are such that the true proportion of success lies in the interval with a confidence of at least a prespecified confidence level $(1-\gamma)100\%$. 
%
The confidence intervals are derived as follows. Let a random variable $X\sim Binomial(n,p)$ where $n$ is the number of observations, each of which has a probability of success $p$. The confidence interval is constructed to bound the value of $p$ with $[\hat{p_l}, \hat{p_u}]$ with prespecified confidence, given $k$ successes in the $n$ observations. The bounds for $p$ are obtained such that the probability of observing more extreme number of successes with the bound value as the probability of success (p-value of the bound) is equal to $\gamma/2$ (Equations~\eqref{eq:lower_pval},\eqref{eq:upper_pval}). This is derived from binomial hypothesis testing where if the p-value falls below a prespecified significance level ($\gamma/2$), then the null hypothesis is rejected. Here, the null hypothesis is for the value of the actual probability of success, and at the values where the p-values reach the significance level we get the lower and upper bounds with confidence $(1-\gamma)$. 
\begin{equation}
    \label{eq:lower_pval}
    Pr\{X\geq k\mid\hat{p_l}\} = \frac{\gamma}{2}
\end{equation}
\begin{equation}
    \label{eq:upper_pval}
    Pr\{X\leq k\mid\hat{p_u}\} = \frac{\gamma}{2}
\end{equation}
A random variable $Z$ following the beta distribution with parameters $a, b\in\mathbb{N}\setminus\{0\}$ has cumulative density function given by Equation~\eqref{eq:beta}. The bounds $\hat{p_l}$ and $\hat{p_u}$ can be obtained from Equations~\eqref{eq:lower_pval},\eqref{eq:upper_pval}, as Beta distribution quantiles with $a=k, b = n-k+1$ (Equation~\eqref{eq:betaquantiles}). 
\begin{equation}
    \label{eq:beta}
    F_Z(p) = Pr\{Z < p\} = \frac{\int_0^pz^{a-1}(1-z)^{b-1}dz}{\int_0^1z^{a-1}(1-z)^{b-1}dz}
\end{equation}
\begin{equation}
    \label{eq:betaquantiles}
    Pr\{Z < p\} = Pr\{X\geq k\mid p\} 
\end{equation}

Thus, $\hat{p_l}=F_{Z_l}^{-1}\left(\frac{\gamma}{2}\right)$ and $\hat{p_u}=F_{Z_u}^{-1}\left(1-\frac{\gamma}{2}\right)$ where $Z_l=Beta(k,n-k+1)$ and $Z_u=Beta(k+1,n-k)$. The obtained interval $\mathcal{I}_{CP}=[\hat{p_l}, \hat{p_u}]$ is such that $Pr\{p\in\mathcal{I}_{CP}\}\geq (1-\gamma)$. 


In the case of bias certification, success corresponds to obtaining an unbiased set of responses from the target LLM $\llm$ for a randomly selected set of prompts from the prompt distribution $\dist(\prompts_0,\attr)$. 
The binomially distributed random variable, whose success probability is determined using confidence intervals is defined as the success count in a set of $\numtrials$ observations made with randomly selected sets of prompts from $\dist(\prompts_0,\attr)$. Thus, in Equation~\eqref{eq:certprob}, the probability term corresponds to the probability of success, for which we construct Clopper-Pearson confidence intervals and compare them with the threshold. Specifically, we compare the lower bound $\hat{p_l}$ with the threshold $1-\eta$ and if  $\hat{p_l}>1-\eta$, we judge $\llm$ to be unbiased with confidence $1-\gamma$. If, however, the upper bound  $\hat{p_u}<1-\eta$, then we judge $\llm$ to be biased with confidence $1-\gamma$. If neither case is true, we continue sampling more sets of prompts and computing confidence intervals till a prespecified upper bound on the number of samples. If the certification does not conclude by then, we declare it inconclusive. 

\subsection{Certification instances}
We certify $\llm$ locally with respect to a single prompt $\prompts_0$, which has been suitably modified to yield a base prompts set $\prompts$, each corresponding to a particular sensitive attribute from $\attr$. For example, for the bias certification with respect to binary gender, we modify the base prompt $\prompts_0$ to assume a male or a female subject. We sample different prompt sets from a distribution that corresponds to adding different prefixes to the base prompt set. 
We certify with respect to 2 types of prefixes: random strings of tokens of a given length and combinations of several jailbreak prefixes. Intuitively, the certificate for the first prefix type is for the bias in the target LLM for any prompting scheme that prepends $\prefixlen$, while that for the second prefix type is for the bias for a prompting scheme that combines common prefixes that effectively jailbreak popular LLMs. 

For the second type of certificate, we combine jailbreaks with probabilistic crossovers and mutations. We start with a main effective jailbreak that can make the target LLM bypass its alignment $\jb_0$. We collect a set of other jailbreak prefixes $\jb = \{\jb_1,\dots\jb_{\helperjbnum}\}$ which are split into individual jailbreak instructions and are crossed-over with $\jb_0$. Each jailbreak instruction from the helper jailbreaks is inserted between the instructions of $\jb_0$ with probability $\crossoverprob$ and is randomly permuted on insertion with other inserted instructions, to constitute the cross-over operation. The mutation operation, that happens after the cross-over, constitutes changing each token of the obtained prefix after cross-over to another randomly selected token, with a probability $\mutprob$. Intuitively, this certification is meant to highlight the potential of combining jailbreaks in bringing out the bias in LLMs. 
